Textualize Visual Prompt for Image Editing via Diffusion Bridge

Visual prompt, a pair of before-and-after edited images, can convey indescribable imagery transformations and prosper in image editing. However, current visual prompt methods rely on a pretrained text-guided image-to-image generative model that requires a triplet of text, before, and after images for retraining over a text-to-image model. Such crafting triplets and retraining processes limit the scalability and generalization of editing. In this paper, we present a framework based on any single text-to-image model without reliance on the explicit image-to-image model thus enhancing the generalizability and scalability. Specifically, by leveraging the probability-flow ordinary equation, we construct a diffusion bridge to transfer the distribution between before-and-after images under the text guidance. By optimizing the text via the bridge, the framework adaptively textualizes the editing transformation conveyed by visual prompts into text embeddings without other models. Meanwhile, we introduce differential attention control during text optimization, which disentangles the text embedding from the invariance of the before-and-after images and makes it solely capture the delicate transformation and generalize to edit various images. Experiments on real images validate competitive results on the generalization, contextual coherence, and high fidelity for delicate editing with just one image pair as the visual prompt.

==> figs/dac.tex <==
\begin{figure*}[t] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering 
\includegraphics[width=1\textwidth]{figs/figure2.pdf} 
\caption{\textbf{Differential attention control}. The attention of the before-image $M_t^b$ is first timed with the column-transformation matrix $\mathbf{\Lambda}$ to switch the column of <end> token, then masked with $\mathbf{F}$. The attention of the after-image $M_t^a$ is masked with $1-\mathbf{F}$ to get the attention of the $y$ tokens. The final $M_t$ is the addition of two masked attentions. This preserves the linguistic format of the cross-attention.} 
\label{dac}
\end{figure*}


==> secs/analysis2.tex <==
\subsection{Ablation and Analysis}
\label{sec:abla}

\noindent\textbf{Differential attention control.} 
The differential attention control injects the attention of the before-image into that of the after-image. We validate its two types of benefits with experiments in Fig.~\ref{dac_abla}. First, during training, the injected attention preserves the invariance making the text embedding better fit on the after-image. As shown in Fig~\ref{dac_abla} 2nd column, the model can better fit the edited dog portrait with the attention injected during the training. Without this, the dog portrait is coarse and lacks details. The text embedding focuses more on learning the transformation and has better generalization ability. Second, during testing, the module can preserve the invariance from the before-image and achieve high fidelity. In 4\&5 columns, with the attention module, the learned text embedding generalizes to edit different images with high fidelity. Without it, the outputs are distorted, meaning that the text embedding overfits the training image pair.


\begin{figure}
\centering
\includegraphics[width=0.42\textwidth]{figs/dac_abla.pdf} 
\caption{\textbf{Train and test results with/without attention}. 1st column: the visual prompt; 2nd column: training results without/with injected attention. 3rd column: test images; 4\&5 columns: test results without and with attention control.} 
\label{dac_abla}
\end{figure}
\begin{figure}
\centering
\includegraphics[width=0.42\textwidth]{figs/ablation2.pdf} 
\caption{\textbf{The predicted $\mathbf{x}_0$ at different timesteps}. The results of early steps without scaling are closer to $\mathbf{x}_0^b$ but the final output deviates. With scaling, the results of early steps are farther but the final output approaches $\mathbf{x}_0^b$.} 
\label{scale}
\end{figure}


\noindent\textbf{Time-aware scaling loss.} We analyzed the predicted $\mathbf{x}_0$, $\mathbf{f}_\theta( \mathbf{x}_{t}, t )$ along all timesteps. The empirical observation in Fig.~\ref{scale} shows that equally optimizing the loss at each timestep may reduce the loss of predicted $\mathbf{x}_0$ in the early steps too much and make the final output deviate from the ground truth $\mathbf{x}_0^a$. Meanwhile, the output that is closest to $\mathbf{x}_0^a$ appears earlier and the image quality degrades undesirably. After scaling, the final output becomes the one closest to $\mathbf{x}_0^a$, and the image quality also improves.




\noindent\textbf{Limitation.} 
One limitation is the prior of the T2I model. Though we leverage the most general T2I model with a large prior, editing real images is still challenging since there are many practical transformations out of the prior of the model. Learning visual prompts is essentially a process of extracting and composing the prior of the text-to-image. Such prior restricts our method to learning visual prompts and editing for real images. Another limitation is choosing the timestamp of the attention injection for different types of editing since the invariance of them is different, to better fit the transformation, we need to choose the appropriate timestep to inject attention for each type of editing in training.














==> secs/supp_checklist.tex <==
\clearpage
\section{Reproducibility Checklist}
This paper:

\noindent 1. Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)

\noindent 2. Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)

\noindent 3. Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes)

\noindent 4. Does this paper make theoretical contributions? (no)

\noindent If yes, please complete the list below.

\noindent 5. All assumptions and restrictions are stated clearly and formally. (yes/partial/no)

\noindent 6. All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)

\noindent 7. Proofs of all novel claims are included. (yes/partial/no)

\noindent 8. Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)

\noindent Appropriate citations to theoretical tools used are given. (yes/partial/no)

\noindent 9. All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)

\noindent 10. All experimental code used to eliminate or disprove claims is included. (NA)

\noindent 11. Does this paper rely on one or more datasets? (no)

\noindent If yes, please complete the list below.

\noindent 12. A motivation is given for why the experiments are conducted on the selected datasets (NA)

\noindent 13. All novel datasets introduced in this paper are included in a data appendix. (NA)

\noindent 14. All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (NA)

\noindent 15. All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)

\noindent 16. All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)

\noindent 17. All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes)

\noindent 18. Does this paper include computational experiments? (yes)

\noindent If yes, please complete the list below.

\noindent 19. Any code required for pre-processing data is included in the appendix. (NA).

\noindent 20. All source code required for conducting and analyzing the experiments is included in a code appendix. (no)

\noindent 21. All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)

\noindent 22. All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes)

\noindent 23. If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)

\noindent 24. This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names, and versions of relevant software libraries and frameworks. (yes)

\noindent 25. This paper formally describes the evaluation metrics used and explains the motivation for choosing these metrics. (yes)

\noindent 26. This paper states the number of algorithm runs used to compute each reported result. (yes)

\noindent 27. Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)

\noindent 28. The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes)

\noindent 29. This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes)

\noindent 30. This paper states the number and range of values tried per (hyper-) parameter during the development of the paper, along with the criterion used for selecting the final parameter setting. (yes)
